A Multimodal Corpus for Emotion Recognition in Sarcasm

While sentiment and emotion analysis have been studied extensively, the relationship between sarcasm and emotion has largely remained unexplored. A sarcastic expression may have a variety of underlying emotions. For example, "I love being ignored" belies sadness, while "my mobile is fabulous with a battery backup of only 15 minutes!" expresses frustration. Detecting the emotion behind a sarcastic expression is non-trivial yet an important task. We undertake the task of detecting the emotion in a sarcastic statement, which to the best of our knowledge, is hitherto unexplored. We start with the recently released multimodal sarcasm detection dataset (MUStARD) pre-annotated with 9 emotions. We identify and correct 343 incorrect emotion labels (out of 690). We double the size of the dataset, label it with emotions along with valence and arousal which are important indicators of emotional intensity. Finally, we label each sarcastic utterance with one of the four sarcasm types-Propositional, Embedded, Likeprefixed and Illocutionary, with the goal of advancing sarcasm detection research. Exhaustive experimentation with multimodal (text, audio, and video) fusion models establishes a benchmark for exact emotion recognition in sarcasm and outperforms the state-of-art sarcasm detection. We release the dataset enriched with various annotations and the code for research purposes: https://github.com/apoorva-nunna/MUStARD_Plus_Plus

==> 0-abstract.tex <==
\begin{abstract}
    While sentiment and emotion analysis have been studied extensively, the relationship between sarcasm and emotion has largely remained unexplored. A sarcastic expression may have a variety of underlying emotions. For example, “I love being ignored” belies sadness, while “my mobile is fabulous with a battery backup of only 15 minutes!” expresses frustration. Detecting the exact emotion behind a sarcastic expression is non-trivial yet an important task. We undertake the task of detecting the exact \textit{emotion in a sarcastic statement}, which to the best of our knowledge is hitherto unexplored. We start with the recently released multimodal sarcasm detection dataset (MUStARD) pre-annotated with 9 emotions. We identify and correct 340 incorrect emotion labels (out of 690). We double the size of the dataset, label with emotions along with \textit{valence} and \textit{arousal} which are important indicators of emotional intensity. Finally, we label each sarcastic utterance with one of the four sarcasm types - \textit{Propositional}, \textit{Embedded}, \textit{Likeprefixed} and \textit{Illocutionary}, with the goal of advancing sarcasm detection research. Exhaustive experimentation with multimodal (text, audio and video) fusion models establishes a benchmark for exact emotion recognition in sarcasm, and outperforms the state-of-art sarcasm detection. We release the dataset enriched with various annotations for research purposes.
\end{abstract}
